Explaining Ontology-Mediated Query Answers using Proofs over Universal Models (Technical Report)

In ontology-mediated query answering, access to incomplete data sources is mediated by a conceptual layer constituted by an ontology, which can be formulated in a description logic (DL) or using existential rules. In the literature, there exists a multitude of complex techniques for incorporating ontological knowledge into queries. However, few of these approaches were designed for explainability of the query answers. We tackle this challenge by adapting an existing proof framework toward conjunctive query answering, based on the notion of universal models. We investigate the data and combined complexity of determining the existence of a proof below a given quality threshold, which can be measured in different ways. By distinguishing various parameters such as the shape of the query, we obtain an overview of the complexity of this problem for several Horn DLs.

==> cq-results.tex <==
% !TEX root = main.tex
% \subsection{The Complexity of Finding Good Proofs in a CQ Derivation Structure}

For example, the arguments in the proof of Theorem~\ref{th:TheACzero} apply in the same way here, \ie one only has to consider constantly many ABoxes (modulo isomorphisms) to search for proofs below a given size bound, and similarly for Theorem~\ref{th:TheACzeroRewritable}.
%
Lemma~\ref{lem:proof-size} also holds for~\Rcq because of Lemma~\ref{lem:transformation}, which gives us the upper bound in Theorem~\ref{th:TheNPDLLite}.
%
Moreover, Lemma~\ref{lem:transformation} also ensures that the arguments for \NP-hardness in Theorem~\ref{th:TheNPDLLite} can be transferred to~\Rcq.

Theorem~\ref{the:el-bounds} allows us to restrict ourselves to
derivation structures of exponential size, which by Lemma~\ref{lem:transformation} also applies to $\Rcq$, \ie $\OP\cq\bin(\EL,\m)$ is in \NExpTime for $\m\in \{\mtree,\msize\}$.

Due to duplication of atoms via~\TAUT, Theorem~\ref{the:np-hard-trees} can also be shown for \Rcq (and so Theorem~\ref{th:ptime-combined} cannot hold for \Rcq):

\begin{restatable}{lemma}{ThmNPHardCQStructure}\label{lem:np-hard-cq-structure}
  For tree-shaped CQs, $\OP\cq(\L,\msize)$ and $\OP\cq(\L,\mtree)$ are \NP-hard.
\end{restatable}
Since domain size is defined in Section~\ref{sec:results} as the number of Skolem terms appearing in a proof, we do not consider it in this section. 
\stefan{TODO: transfer results for \EL and larger logics?}


%\stefan{TODO: copy results from DL paper}

